PaD: Program-aided Distillation Can Teach Small Models Reasoning Better than Chain-of-thought Fine-tuning

While large language models (LLMs) excel in various natural language processing tasks, their huge size and the inaccessibility of parameters present challenges for practical deployment. Previous studies try to distill task-specific ability from LLMs to smaller models, using data synthesis and chain-of-thought (CoT) fine-tuning. However, synthetic CoT data often contains faulty reasoning, which deteriorates the quality of distillation, especially in reasoning capabilities. In this work, we propose Program-aided Distillation (PaD), which introduces reasoning programs to suppress the errors in distilled data, and thus achieves better distillation quality for reasoning tasks. In PaD, we utilize the reasoning program to substitute the CoT, allowing automated error checking of synthetic data. Further, through error injecting and further training, the small distilling model could iteratively self-refine the reasoning. Moreover, we conduct a step-wise beam search by step-by-step verifying to acquire more exact reasoning chains. We evaluate PaD on arithmetic reasoning, symbolic reasoning, and general ability. Experimental results demonstrate that smaller models using PaD can not only outperform certain LLMs~(e.g., LLaMA-1 13B) but also achieve strong improvement over baselines with a significantly smaller scale of parameters and data. The source code is publicly available at https://github.com/Xuekai-Zhu/pad.

==> sections/results.tex <==
\section{Results}

\begin{figure*}[t!] 
\centering 
\includegraphics[width=0.98\linewidth]{figures/ablation.pdf} 
\caption{The ablation of PaD. Comparing with standard fine-tune and the base model, PaD achieves significant mathematical reasoning improvement. However, PaD brings a noted trade-off in general capabilities. Based on PaD, self-distillation can also provide a minor boost.}
\label{fig:ablation} 
\end{figure*}

\begin{figure}[t!] 
\centering 
\includegraphics[width=0.95\linewidth]{figures/data_pruning.pdf} 
\caption{The performance under different data pruning metrics.}
\label{fig:data_pruning} 
\end{figure}


\begin{figure}[t!] 
\centering 
\includegraphics[width=0.95\linewidth]{figures/gramma_correct.pdf} 
\caption{Comparing grammatically correct rate trained by different fraction of data. These data was re-ordered by GraNd~\cite{paul2021deep}. Under 50\% data pruning, CodeT5\_base achieves comparable accuracy with~\texttt{gpt-3.5-turbo}. This demonstrates that program-aided format is suitable for small models.}
\label{fig:gramma_correct} 
\end{figure}

\begin{figure}[t!] 
\centering 
\includegraphics[width=0.95\linewidth]{figures/chatgpt_eval_acc.pdf} 
\caption{The evaluation of data synthesis on train and test set of GSM8K. Success refers to correct compilation and answer. Miscalculation indicates correct compilation but an incorrect answer.}
\label{fig:chathpt_eval_acc} 
\end{figure}

\begin{figure}[t!] 
\centering 
\includegraphics[width=0.95\linewidth]{figures/chatgpt_eval.pdf} 
\caption{The evaluation of semantic consistency, logicality and informativeness of synthetic data. Here, four different contexts used for data synthesis. We utilize the metric suite from~\cite{golovneva2023roscoe}. The results illustrated \texttt{gpt-3.5-turbo} can synthesize high-quality data with rare repetition and high faithfulness in reasoning steps. The detailed contexts shown in Appendix~\ref{sec:context_example}.
}
\label{fig:chathpt_eval} 
\end{figure}





